Practical Bayesian Optimization of Objectives with Conditioning Variables

Bayesian optimization is a class of data efficient model based algorithms typically focused on global optimization. We consider the more general case where a user is faced with multiple problems that each need to be optimized conditional on a state variable, for example given a range of cities with different patient distributions, we optimize the ambulance locations conditioned on patient distribution. Given partitions of CIFAR-10, we optimize CNN hyperparameters for each partition. Similarity across objectives boosts optimization of each objective in two ways: in modelling by data sharing across objectives, and also in acquisition by quantifying how a single point on one objective can provide benefit to all objectives. For this we propose a framework for conditional optimization: ConBO. This can be built on top of a range of acquisition functions and we propose a new Hybrid Knowledge Gradient acquisition function. The resulting method is intuitive and theoretically grounded, performs either similar to or significantly better than recently published works on a range of problems, and is easily parallelized to collect a batch of points.

==> secs/4-con_v_global.tex <==
\section{Risks in Conditional Optimization}
\textbf{Policy optimization vs data optimization:} 
Consider the case where the number of states, $N_s$, is 
significantly smaller than the sampling budget $N_s\ll N$. If many
states are very similar, an algorithm learning the optimal action
for each state, $\argmax_x \E[ f(s,x)]$ or \emph{policy optimization},
may intentionally ignore some states, $s_{i}$, if $\argmax_x \E[ f(s_{i},x)]$ is accurately known
due to many samples on surrounding states $s_{s}$, saving valuable samples for less clustered states.
However, for a user that wants to find good observations $\max y$ for each state,
or \emph{data optimization},
states $s_i$ will have very few observations and therefore rather poor $\max y$.
\cite{pearce2018continuous} suggested performing
data efficient policy optimization first and reserving the final $N_s$ 
for data optimization,
allocating one sample per state with the action
determined by EI yielding better performance
than using EI throughout. Alternatively, using MTS provides a
compromise between policy and data optimization and showed 
mixed or better results than risk-averse REVI for data optimization.
% In general in the small state setting, 
% these are competing goals and an algorithm must be designed
% with the goal in mind. In stochastic simulation optimization, 
% a user is only interested in policy optimization; the best action
% will be deployed for long term use and stochastic realizations of
% $\max y$ observed during optimization are not 
% the true long term reward $\E[f(s, \pi(s))]$. 
% In
% machine learning, a user is more interested in data optimization,
% finding a trained model that performs well because the resulting
% model will be deployed for future use (not necessarily the
% hyper-parameters/actions used to train it). 
Global optimisation may be viewed as one state that receives \emph{all} data points.

\textbf{Additive kernels:} \cite{kandasamy2015high}
\cite{krause2011contextual} suggest using
additive kernels for higher dimensional domains
and for contextual optimization.
Such kernels assume the function being modelled decomposes into
a sum of functions, each one depending on an exclusive subset of variables.
If the state variables and action variables are not in the same subsets
then the assumed structure, $f(s, x) = g(s) + h(x)$,
is reflected in the mean function $\mu^n(s, x) = \mu^n_1(s) + \mu^n_2(x)$ and
$$
\pi(s) = \argmax_x \mu^n(s, x) = \argmax_x \mu_1^n(x).
$$
The recommended action is \emph{independent of state}, no method can
learn the optimal action for each state. In general, additive structure
assumes \emph{no interaction} between variables, conditional
optimization is only necessary \emph{with interaction} between variables.
Hence for higher dimensional problems, $\CONBO$ can be applied to the
subset of interacting state-action variables with the rest fixed.


\textbf{State boundary effects:}\label{sec:state_boundary_effects}
collecting data at a given $(s,x)\n1$ point, total benefit is integrated
over states. When using a stationary kernel, if $s\n1$ is on the boundary
of state space, many nearby affected states lie outside feasible state space
and the integral over states is reduced. For example, optimizing the warehouse
with maximum demand helps to learn optimal stock only for warehouses with lower demands
whereas optimizing the warehouse with large demand, but not maximum, helps medium 
large and maximum demand warehouses. With
higher state dimension, this effect becomes more and more significant as there
are more state boundaries and high dimensional corners with exponentially
fewer neighboring states. This effect is accounted for by acquisition 
functions that integrate over states like \CONBOt and REVI, but not for
methods like SCoT, PEI, PEQI or MTS.
% When using a product kernel $k(s,x,s',s')=k_s(s,s')k_x(x,x')$,
% this state boundary effect may be simulated by applying a convolution operation to the state
% density $\tilde P[s] = \int_s\P[s']k(s,s')ds$ 

==> sm_secs/3-global-on-conditional.tex <==
\section{Global algorithms on conditional problems}
Note that state is determined by the algorithm. 
Global optimization algorithms prioritize sampling state-action pairs
with high reward while conditional algorithms prioritize sampling states with high
density and actions with high reward. Thus, if high reward states coincide with high density states, both algorithm types will behave similarly. The ambulance problem may be an instance of this special edge case
as state density is peaked in the centre of the map where journey times may also be
minimized. We have added this hypothesis to the paper and leave a fuller study of
such subtle edge case test problems to future work. Further, R1 commends the inclusion of EI.

% Hence the anomalous EI result may expose a feature of
% the problem and not a feature of the algorithm.

\begin{figure}
\label{fig:synth}
    \centering
    \includegraphics[width=0.75\textwidth]{sm_pics/state-mult-lambda0-3algos.pdf}
\end{figure}

To demonstrate the necessity of conditional methods,
we apply EI, hybrid KG and ConBO
to a range of synthetic conditional problems that vary only by the width of the state
space. Zero width means that state space is a single state, the problem
reduces to global optimization and all methods achieve
near zero OC. As width increases to 1 (full state space), there are more states to optimize and
ConBO optimizes each state consistently achieving near zero OC while
EI and KG do not optimize every state and do not converge (see Figure \ref{fig:synth}). We have included this experiment and discussion in the paper.

==> sm_secs/Compare-REVI-MTS.tex <==
\section{Relation to Previous Methods}
\subsection{REVI}

\begin{itemize}
    \item scaling with dimension
    \item discretization fixed with x^n+1
    \item deteministic optimizer, bias
    \item sparsity trick and convolution trick
    \item 
\end{itemize}

At each iteration the REVI algorithm discretizes the states space $S$ with samples from $\P[s]$ and the action
space with uniform random samples over $X$, the cross product of these sets forms a discretization over the full
state-action domain. Hence, for each state the KG by discretization may be used and the average over states
approximates the total benefit of a new sample. While this method is simple to compute, it suffers multiple
drawbacks that restrict its applicability.

Firstly the curse of dimensionality. With increasing state space
and action space the discretization size must grow exponentially. In the REVI algorithm, the discretization
is frozen and kept constant for each iternation, this allows various computations to be precomputed and cached.
However with exponentially increasing discretization, this corresponds to
exponentially increasing memory requirement. Instead of caching, quantities may be computed on demand and discarded
which reduces memory requirement but then requires exponential time to compute quantities over an exponential
number of points in the discretization. In our implementation, we occasionally found that REVI would run out of memory
and experiments would crash and thus we had to reduce discretization size.

Secondly, discretizing the state space and optimizing an average over discrete states is a biased estimate of the 
true benefit across the infinite continuum of states. In the REVI framework, this can only be remedied by increasing
samples size thereby increasing the discretization. If the sample size is too small, The Monte-Carlo estimate
is poor, if the sample size is large, the algorithm complexity grows as described above.

Thirdly, the algorithm is sensitive to hyperparameters. If the state space discretreization is too low, small $n_s$, 
then a sample at $(s,x)\n1$ may have few or no neighboring states over which to measure the benefit. If the action space
discretization is too small, then for each state, Knowledge Gradient by discretization will be very poor estimate of the
benefit of a new point on that state. Again, in the REVI framework, these can only be remedied by increasing
discretization sizes. In general, if the typical distance between points in the discretization is comparable or
longer than the length scales of the GP model, then REVI acquisition function becomes random.
If the interpoint spacing is much larger, computation significantly slows down.


The ConBO framework does not suffer any of these issues. Firstly, the Monte Carlo integration over states is
stochastic with each call to ConBO. By using the Adam optimizer, the peak that is found at the
end of optimizing ConBO$(s,x)$$ is an unbiased estimate of the true average over infinitely many states.

Secondly, ConBO uses importance sampling, the Monte-Carlo states depend upon $(s,x)\n1$ such that only very
relevant states within GP length scales of $(s,x)\n1$ are included in the integration, thereby reducing variance,
improving approximation accuracy and the convergence of the Adam optimizer.

Thirdly, by using the hybrid KG approach, the benefit of a sample on one state can be estimated very accurately
regardless of the dimensionallity of the action space $X$, one may use $n_z=5$ for any dimensional space and
the {\tt Optimizer}$(\cdot)$ uses gradients and convergence does not scale exponentially with .

In summary, both methods use similar motivation, however REVI is biased, sensitive to hyperparameters
either resulting in poor approximations if the hyperparameters are too low or expensive computation
if they are too high. As a result, REVI can be safely applied in low dimensional simple problems, 
however the algorithm performance becomes very unstable for larger problems. 

ConBO, with stochastic integration and stochastic gradient ascent, importance sampling over states, and
hybrid KG over actions does not suffer these problems and therefore performs much mre reliably over
the range of problems considered.
